A Systematic Study of Knowledge Distillation for Natural Language Generation with Pseudo-Target Training

Modern Natural Language Generation (NLG) models come with massive computational and storage requirements. In this work, we study the potential of compressing them, which is crucial for real-world applications serving millions of users. We focus on Knowledge Distillation (KD) techniques, in which a small student model learns to imitate a large teacher model, allowing to transfer knowledge from the teacher to the student. In contrast to much of the previous work, our goal is to optimize the model for a specific NLG task and a specific dataset. Typically in real-world applications, in addition to labeled data there is abundant unlabeled task-specific data, which is crucial for attaining high compression rates via KD. In this work, we conduct a systematic study of task-specific KD techniques for various NLG tasks under realistic assumptions. We discuss the special characteristics of NLG distillation and particularly the exposure bias problem. Following, we derive a family of Pseudo-Target (PT) augmentation methods, substantially extending prior work on sequence-level KD. We propose the Joint-Teaching method, which applies word-level KD to multiple PTs generated by both the teacher and the student. Finally, we validate our findings in an extreme setup with no labeled examples using GPT-4 as the teacher. Our study provides practical model design observations and demonstrates the effectiveness of PT training for task-specific KD in NLG.

==> tables/kd.tex <==
\def\arraystretch{0.85}
\begin{table}
\centering
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{l|cccc|c|c}

\toprule
A. \textbf{Objective} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} & \textbf{Wins} & \textbf{Dev} \\
  & (\%) & (\%) & (\%) & (\%) & &\\
\midrule
 Fine-tune & 0.0 & 0.0 & 0.0 & 0.0 & 0 & 14.8 \\
 Logits & \textbf{36.6} & \textbf{37.9} & \textbf{35.1} & 28.0 & 13 & \textbf{16.0} \\
 Noisy & 28.3 & 36.4 & 33.3 & \textbf{46.6} & \textbf{14} & 15.9 \\
 Att-Rel & 23.0 & 28.1 & 24.3 & 25.3 & 5 & 15.9 \\

\midrule
 B. \textbf{PTs} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} & \textbf{Wins} & \textbf{Dev} \\
\midrule
Logits & 36.6 & 37.9 & \textbf{35.1} & \textbf{28.0} & 10 & 16.0 \\
Seq-lvl & 23.4 & 23.1 & 12.2 & -45.7 & 0 & 15.7 \\
Logits+Seq & \textbf{39.8} & \textbf{40.8} & 32.7 & 27.6 & \textbf{22} & \textbf{16.3} \\

\midrule
 C. \textbf{Unlabeled} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} & \textbf{Wins} & \textbf{Dev} \\
\midrule
Labeled & 39.8 & 40.8 & 32.7 & 27.6 & 0 & 16.3 \\
 + Unlabeled & \textbf{58.6} & \textbf{64.8} & \textbf{52.8} & \textbf{38.2} & \textbf{32} & \textbf{16.9} \\

\midrule
 D. \textbf{Decoding} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} & \textbf{Wins} & \textbf{Dev} \\
\midrule
 Single PT & 58.6 & 64.8 & 52.8 & 38.2 & 1 & 16.9 \\
 K-Beams & 66.5 & 68.0 & 59.5 & 46.2 & 4 & 17.0 \\
 Sampling & \textbf{68.3} & \textbf{73.1} & \textbf{64.9} & 55.0 & \textbf{15} & \textbf{17.2} \\
 H-Sampling & 67.4 & 69.7 & 63.7 & \textbf{59.8} & 12 & 17.1 \\

\midrule
 E. \textbf{Joint-T} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} & \textbf{Wins} & \textbf{Dev} \\
\midrule
 Only Teacher & 68.3 & 73.1 & 64.9 & 55.0 & 4 & 17.2 \\
 Only Student & 65.1 & 71.0 & 65.7 & 54.0 & 3 & 17.1 \\
 Joint-Teaching & \textbf{75.1} & \textbf{78.1} & \textbf{70.9} & \textbf{59.2} & \textbf{25} & \textbf{17.4} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Average fractions of the student-teacher {\em performance gaps closed} by different KD methods, number of winning setups (out of 32) and development scores. Table A: KD objectives (S3); Table B: PT augmentation (S4). Table C: PTs for unlabeled examples (S5); Table D: Decoding methods for generating PTs (S6+S7); Table E: PTs generated only by the teacher, the student, or Joint-Teaching (S8). For more details about the methods see \S\ref{sec:methods} and \S\ref{sec:formal_methods}. Metrics: BLEU (BL), ROUGE (RG), BertScore (BS), Perplexity (PP).}
\label{tab:kd}
\vspace{-1em}
\end{table}

==> tables/kd_gpt.tex <==
\def\arraystretch{0.9}
\begin{table}
\centering
\begin{adjustbox}{width=0.47\textwidth}
\begin{tabular}{l|p{0.4cm}p{0.4cm}p{0.4cm}p{0.6cm}|p{0.4cm}p{0.4cm}p{0.4cm}p{0.6cm}}
\toprule
  & \multicolumn{4}{c|}{\squad{}} & \multicolumn{4}{c}{\shakespeare{}} \\
\textbf{Method} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} \\
\midrule
 a. GPT-4 & 13.6 & 37.6 & 75.0 & & 21.4 & 42.3 & 79.4 & \\
 b. GT labels  & 17.8 & 36.4 & 75.2 & 2.1 & 21.2 & 42.1 & 76.4 & 2.1  \\
 \midrule
 c. Single PT & 11.7 &       32.6 &              72.4 &    2.65 &           18.9 &       \textbf{41.1} &              76.0 &    2.47 \\
 d. Multiple PTs &  11.6 &       32.7 &              72.4 &    2.84 &           \textbf{19.2} &       \textbf{41.1} &              \textbf{76.1} &    \textbf{2.36}  \\
 e. Logits + PT & 11.6 &       32.4 &              72.4 &    2.72 &           18.5 &       41.0 &              75.9 &    2.66 \\
 f.  Logits + PTs & \textbf{11.9} &       \textbf{32.8} &              \textbf{72.5} &    \textbf{2.48} &           19.1 &       40.7 &              75.0 &    2.52 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Average \textbf{BL}EU, \textbf{R}OU\textbf{G}E, \textbf{B}ERT\textbf{S}core and \textbf{PP}L scores of different methods in the extreme setup. }
\label{tab:kd_gpt}
\vspace{-1em}
\end{table}

==> tables/models.tex <==
\begin{table}
\centering
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{l|cccc|cccc}
\toprule
 \textbf{Model} & \textbf{\#P} & \textbf{\#F} & \textbf{Lat} & \textbf{Thr} & \textbf{BL} & \textbf{RG} & \textbf{BS} & \textbf{PP} \\
\midrule
 \underline{\tfivel} & 737 & 19.5 & 597 & 5.3 & 16.4 & 34.6 & 75.1 & 1.6  \\
 \textbf{\tfives}  & 60 & 1.4 & 160 & 55.2 & 13.4 & 30.8 & 72.7 & 2.4 \\

% \emph{\tfivekd} & 6-6 & (-92\%) & (-93\%) & (x3.7) & (x10.4) & 15.5 (71\%) & 33.5 (72\%) & 74.3 (67\%) & 1.9 (63\%) & 17.2 \\
 \midrule
 
 \underline{\bartl} & 406 & 10.0 & 281 & 7.8 & 16.4 & 34.8 & 75.4 & 1.7  \\
 \bartb & 139 & 3.0 & 147 & 13.5 & 14.5 & 32.7 & 74.2 & 1.9  \\
 \bartp & 111 & 1.7 & 146 & 16.0 & 11.4 & 28.0 & 71.6 & 2.2  \\
 \textbf{\barts} & 407 & 2.6 & 75 & 15.3 & 13.3 & 31.5 & 73.3 & 2.6  \\

% \emph{\bartkd} & 6-2 & (-75\%) & (-74\%) & (x3.7) & (x2.0) & 15.8 (80\%) & 34.2 (82\%) & 75.0 (80\%) & 2.0 (62\%) & 17.6 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{A comparison between different ED models based on stages 1 and 2 (only fine-tuning, no KD). All measures are the average over four NLG tasks. Parameters (\#P) are in millions, FLOPs (\#F) are in billions, Latency (Lat) is in milliseconds, Throughput (Thr) is in thousands of examples per minute, both are measured on an Nvidia GeForce RTX 4080. 
We also indicate the participating models in the KD stages (3-8): Teachers are underlined, student baselines (no KD) are in bold.}
\label{tab:models}
\vspace{-1em}
\end{table}
